Representational Systems Theory: A Unified Approach to Encoding, Analysing and Transforming Representations

The study of representations is of fundamental importance to any form of communication, and our ability to exploit them effectively is paramount. This article presents a novel theory -- Representational Systems Theory -- that is designed to abstractly encode a wide variety of representations from three core perspectives: syntax, entailment, and their properties. By introducing the concept of a construction space, we are able to encode each of these core components under a single, unifying paradigm. Using our Representational Systems Theory, it becomes possible to structurally transform representations in one system into representations in another. An intrinsic facet of our structural transformation technique is representation selection based on properties that representations possess, such as their relative cognitive effectiveness or structural complexity. A major theoretical barrier to providing general structural transformation techniques is a lack of terminating algorithms. Representational Systems Theory permits the derivation of partial transformations when no terminating algorithm can produce a full transformation. Since Representational Systems Theory provides a universal approach to encoding representational systems, a further key barrier is eliminated: the need to devise system-specific structural transformation algorithms, that are necessary when different systems adopt different formalisation approaches. Consequently, Representational Systems Theory is the first general framework that provides a unified approach to encoding representations, supports representation selection via structural transformations, and has the potential for widespread practical application.

==> background.tex <==

To exemplify representation choices, we present a problem and different ways in which it can be expressed and solved. The scope of these representations, and thus the representational systems from which they are drawn, is large, including natural language (NL), formal notation, a geometric figure, and a table. This variety illustrates the breadth of representations to which our theory can be applied and provide just one context in which re-representation can be desirable. So, suppose that we have a representation drawn from a natural language system, which could readily be presented in a lecture on probability\footnote{We previously published this example in~\cite{raggi2020re}.}:

\begin{paragraph}{Medical Test Problem} Suppose that 4\% of the population has a disease~$D$. For those who have the disease, a test $T$ is accurate 95\% of the time. For those who do not have the disease, $T$ is accurate 90\% of the time. If you take the test and it comes out positive, what is the probability that you have the disease?
\end{paragraph}
%

There are many other representations of this problem, drawn from various representational systems. Each of these alternative systems has different entailment relations and, thus, different mechanisms can be used to solve the problem. The choice of representation may depend on the ability of the students, their prior knowledge, or their own cognitive biases. An effective choice could better support their learning, or ability to solve the problem: it is well-known that representation choice in mathematics is an important factor in students' progress~\cite{doi:10.1080/10986061003654240}. For the purposes of illustration, we present three of these alternatives.

\newcommand{\Prob}{\textup{P}}
\begin{paragraph}{Bayesian Representation}
It is given that $\Prob(D)\!=\!0.04$, $\Prob(T\! \mid \! D)\! = \!0.95$, $\Prob(\overline{T}\! \mid \! \overline{D})\! =\! 0.9$. What is  $\Prob(D\!\mid\! T)$?
\end{paragraph}
%
%\begin{paragraph}{Bayesian Solution}
%	\begin{align*}
%	\Prob(D \mid T) &= \frac{ \Prob(T | D) \Prob(D)}{ \Prob(T)} \\
%    & = \frac{ \Prob(T \mid D) \Prob(D)}{ \Prob(T \cap D) +  \Prob(T \cap \overline{D})} \\
%	& = \frac{ \Prob(T \mid D) \Prob(D)}{ \Prob(T  \mid  D) \Prob(D) +  \Prob(T  \mid  \overline{D}) \Prob(\overline{D})} \\
%	& = \frac{ \Prob(T \mid D) \Prob(D)}{ \Prob(T  \mid  D) \Prob(D) +  (1-\Prob(\overline{T}  \mid  \overline{D})) (1-\Prob(D))} \\
%	& = \frac{0.95 \cdot 0.04}{0.95 \cdot 0.04 + (1- 0.9) \cdot (1-0.04)}
%	\approx 0.28
%	\end{align*}
%Hence $\Prob(D\!\mid\! T)\approx 0.28$.
%\end{paragraph}





\begin{paragraph}{Area Diagrams Representation}
Calculate the size ratio between the area of the patterned region, \,\tikz[scale=.25]{\draw[fill=black, fill opacity = 0.55, pattern=north west lines, pattern color=black] (0,0) rectangle (1,1)},\, and the area of the shaded region, \tikz[scale=.25]{\draw[fill=black, fill opacity = 0.15] (0,0) rectangle (1,1)}:\\
\begin{adjustbox}{valign=C}
	%\begin{wrapfigure}{r}{0.33\linewidth}\hspace*{-0.75em}
		\begin{tikzpicture}[scale=1]
		%
		\tikzstyle{every node}=[font=\scriptsize]
		%
		\draw [fill=white] (0, 0) rectangle (2, 2);
		\draw [fill=white] (0, 0) rectangle (0.1, 2);
		\draw [fill=black, fill opacity = 0.15] (0, 0.1) rectangle (0.1, 2);
		\draw [pattern=north west lines, pattern color=black] (0, 0.1) rectangle (0.1, 2);
		\draw [fill=black, fill opacity = 0.15] (0.1, 1.8) rectangle (2, 2);
		%
		%		\node at (.05,-0.19) {$D$};
		%		\node at (1.1,-0.183) {$\overbar{D}$};
		%		\node at (-.2,1.1) {$T$};
		%		\node at (-.2,0.1) {$\overbar{T}$};
		%		\node at (2.2,1.9) {$T$};
		%		\node at (2.2,0.9) {$\overbar{T}$};
		%
		\draw [decorate,decoration={brace,amplitude=5pt,mirror},yshift=0pt]
		(2.05,0) -- (2.05,1.8) node [black,midway,xshift=0.35cm] {\scriptsize\rotatebox[]{270}{$0.9$}};
		%
		\draw [decorate,decoration={brace,amplitude=5pt},yshift=0pt]
		(-0.05,0.1) -- (-0.05,2) node [black,midway,xshift=-0.35cm] {\scriptsize\rotatebox[]{90}{$0.95$}};
		%
		\draw [decorate,decoration={brace,amplitude=0.8pt},yshift=0pt]
		(-0.01,2.05) -- (0.11,2.05) node[black,midway,yshift=0.2cm] {\scriptsize$0.04$};
		%
		\draw [decorate,decoration={brace,amplitude=5pt,mirror},yshift=0pt]
		(-0.01,-0.05) -- (2.01,-0.05) node[black,midway,yshift=-0.35cm] {\scriptsize$1$};
		%		\node at (-.35,0.9) {$t \mid d$};
		%		\node at (-.35,1.9) {$\bar{t} \mid d$};
		%		\node at (2.35,0.1) {$t \mid \bar{d}$};
		%		\node at (2.35,1.1) {$\bar{t} \mid \bar{d}$};
		%
		\end{tikzpicture}\vspace{-1em}
	%\end{wrapfigure}%
	\strut
	%\vspace*{-1ex}
\end{adjustbox}
\end{paragraph}


%\begin{paragraph}{Area Diagrams Solution}
%The area of the patterned rectangle is $0.95\times 0.04$. The area of the two shaded rectangles, (including the patterned region), is $0.95\times 0.04+(1-0.9)\times(1-0.04)$. The ratio of these areas is $\approx 0.28$.
%\end{paragraph}

%

\begin{paragraph}{Contingency Tables Representation}\label{medical-cont} Calculate the ratio of the value of cell $(T,D)$ against $total(T)$.\\
%	\begin{table}[h]\centering
%		\def\arraystretch{1.1}
%		\noindent
% \resizebox{0.8\columnwidth}{!}{
\begin{center}
		\begin{tabular}{|p{0.1\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}|}
			\hline
			& \textbf{$D$} & \textbf{$\overline D$} & \textbf{total} \\
			\hline
			\textbf{$T$} & \cellcolor{gray!20}$0.95 \cdot 0.04$ &  & \cellcolor{gray!20} \\
			\hline
			\textbf{$\overline T$} &  & $0.9\cdot total(\overline D)$ &  \\
			\hline
			\textbf{total} & $0.04$ & & 1 \\
			\hline
		\end{tabular}%}
\end{center}
%	\vspace{-12pt}
%	\end{table}
\end{paragraph}

%\begin{paragraph}{Contingency Tables Solution (sketch)}
%Using the law of total probability, calculate $\operatorname{total}(\overline D)$, followed by the value of cell $(T,\overline{D})$, followed by $\operatorname{total}(T)$. Finally, obtain the desired ratio $\approx$ $0.28$. Complete workings would populate the table with values.
%\end{paragraph}

It is self-evident that these four different representations have fundamentally different syntaxes and by their very nature afford different approaches to solving the medical problem. Representational Systems Theory provides a unified framework that allows each of these representations to be encoding using a graph-theoretic approach. Given higher-level descriptions of the systems from which they are drawn, and suitable links between these descriptions, we are able to transform between these representations. In prior work~\cite{raggi2020re}, we presented a much earlier version of the framework presented here. However, that prior work did not support the identification of new representations in particular. Rather, it sought to address \textit{whether} a representation \textit{could be re-represented} in another representational system. The research in this paper thus represents a substantial advance over our previous contributions.

%We now give a high-level sketch of the structural transformation process that Representational Systems Theory supports. Firstly, we are able to \textit{encode} an initial representation of the problem, using a \textit{construction}. Then, given \textit{patterns} that \textit{describe} constructions in the four representational systems, along with links between patterns, we are able to structurally transform (a construction of) the initial representation into (constructions of) the remaining three representations, using a \textit{structure transfer algorithm}.  This paper specifically demonstrates how to use Representational Systems Theory to \textit{define} a structural transformation relation between representations across representational systems. Omitted from this paper is a detailed algorithm to produce these transformations. Rather, our contribution provides the basis on which such algorithms can be devised. 
